Bimetric interactions based on metric congruences

In massive gravity and bigravity, spin-2 interactions are defined in terms of a square root matrix that involves two metrics. In this work, the interactions are constructed using a congruence matrix between the metrics. It is established that the primary square root matrix function is the only power series solution to the equations of motion for the congruence. Moreover, the shift vector redefinition that is used in the bimetric ghost-free proofs follows from the $N+1$ form of the equations of motion. The analysis also gives an insight into the vielbein formulation of spin-2 interactions since the bimetric formulation in terms of a congruence is algebraically equivalent to the unconstrained vielbein formulation.

==> sec-40.tex <==

\subsection{Note on the vielbein formulation}

Several comments:

The bimetric formulation in terms of a congruence $S$ is algebraically
equivalent to the unconstrained vielbein formulation in terms of the
vielbeins $\gE$ and $\fE$.

The ghost-proof in \cite{Hinterbichler:2012cn} assumes the simultaneous
$N+1$ decomposition with arbitrarily ``boosted'' vielbeins, which
is not possible in general. Namely, we cannot ensure that the vielbein
$\fE$ can simultaneously be triangularized together with $\gE$.
A counterexample is shown in Figure \ref{fig:bad-nc} where the null
cones of the two metrics doubly intersect; in this case the simultaneous
$N+1$ decomposition of $\gMet$ and $\fMet$, and the simultaneous
triangularization of $\gE$ and $\fE$, are not possible.

\begin{figure}[H]
\noindent \begin{centering}
\includegraphics[width=35mm]{fig-2}
\par\end{centering}
\caption{\label{fig:bad-nc}Null cones for the metric configuration which does
not allow a boosted $N+1$ decomposition wherein the both vielbeins
are in the triangular form. }
\end{figure}

In previous arXiv versions of \cite{Hinterbichler:2012cn} (including
the published one), the authors proposed a method of dealing with
the local spatial rotation invariance using constrained spatial vielbeins.
The most recent of the paper (v3) omits two pages on that matter.
The authors justify the removal pointing out in a footnote that it
is not clear that such a method works since solving the constraint
(eq. 2.27 of v2 \cite{Hinterbichler:2012cn}) may introduce dependence
on the lapse or shift into the vielbeins (this remark was first put
forward by Shuang-Yong Zhou). As we have shown, variation with respect
to both $\sLp$ and the rotation resolves this issue and produces
the square root (which is compatible with appendix C in \cite{Hinterbichler:2012cn}).

